Relational World Knowledge Representation in Contextual Language Models: A Review

Relational knowledge bases (KBs) are commonly used to represent world knowledge in machines. However, while advantageous for their high degree of precision and interpretability, KBs are usually organized according to manually-defined schemas, which limit their expressiveness and require significant human efforts to engineer and maintain. In this review, we take a natural language processing perspective to these limitations, examining how they may be addressed in part by training deep contextual language models (LMs) to internalize and express relational knowledge in more flexible forms. We propose to organize knowledge representation strategies in LMs by the level of KB supervision provided, from no KB supervision at all to entity- and relation-level supervision. Our contributions are threefold: (1) We provide a high-level, extensible taxonomy for knowledge representation in LMs; (2) Within our taxonomy, we highlight notable models, evaluation tasks, and findings, in order to provide an up-to-date review of current knowledge representation capabilities in LMs; and (3) We suggest future research directions that build upon the complementary aspects of LMs and KBs as knowledge representations.

==> 02-related.tex <==
% % We briefly overview related survey and position papers from the knowledge bases and language modeling literature. 

% \paragraph{Knowledge bases}
% Research in knowledge bases spans several decades and multiple subfields of computer science. 
% For an up-to-date overview of \kb{}s from \nlp{} and machine learning perspectives, we refer the reader to the  survey by~\citet{weikum-etal-2020-machine}. 
% Most related to our work in terms of scope and topic, 
% \citet{colon-etal-2021-combining} review several works that integrate structured knowledge into \lm{}s, and
% \citet{yu-etal-2020-kenlg-survey} survey  text generation methods that use external knowledge sources, including \kb{}s. 
% \citet{heinzerling-inui-2020-language}  provide a brief table that categorizes \nlp{} approaches to world knowledge representation, including methods that fuse \kb{}s and \lm{}s. 

% \paragraph{Language modeling}
% Several works review the text representation capabilities of the BERT \lm{} specifically, briefly touching on entity- and world-level ``knowledge'' (or semblance thereof) within BERT~\cite{tenney-etal-2019-bert,rogers-etal-2021-primer}. 
% \citet{qiu-etal-2020-survey} survey contextual language models more broadly, including but not limited to those enhanced by \kb{}s. 
% Others reviews cover methodological and ethical concerns related to language modeling, including the lack of grounding~\cite{bender-koller-2020-climbing,bisk-etal-2020-experience}, the environmental costs of deep learning~\cite{strubell-etal-2019-energy,schwartz-etal-2019-green-ai}, and the learning of harmful biases~\cite{bender-etal-2021-stochastic-parrots}. 
% Such arguments may implicitly motivate the usage of \kb{}s to improve the efficiency of \lm{} knowledge acquisition and the quality of such knowledge, although this is neither a focus of the previous works nor our own.


==> 06-eval.tex <==
\begin{table*}[t!]
\centering
\caption{
We ``invert'' the organization here: 
    Common evaluation tasks and benchmarks across all three levels of supervision, with representative examples from the literature. 
}
\label{table:evaluation}
\resizebox{\textwidth}{!}{
    \begin{tabular}{ l p{6cm} c p{5cm} p{5cm} p{5cm} }
    \toprule
    \multicolumn{2}{l}{Evaluation setup} && \multicolumn{3}{l}{Supervision level} \\
    \cline{1-2} \cline{4-6}
    Task & Benchmarks && Token & Entity & Relation \\ 
    \toprule 
    \multirow{3}{*}{Knowledge probing} 
        & LAMA \cite{petroni-etal-2019-language}, LAMA-UHN \cite{poerner-etal-2020-e-bert}, mLAMA \cite{kassner-etal-2021-multilingual}
        && \cite{petroni-etal-2019-language,jiang-etal-2020-how-can,dufter-etal-2021-static}
        & \cite{xiong-etal-2020-pretrained-encyclopedia,fevry-etal-2020-entities,poerner-etal-2020-e-bert} 
        & \cite{agarwal-etal-2021-large} \\
    \midrule 
    \multirow{3}{*}{Entity linking} 
        & AIDA/CoNLL \cite{hoffart-etal-2011-robust},
        TACKBP-2010 \cite{ji-etal-2010-overview},
        zero-shot \cite{logeswaran-etal-2019-zero}
        &&
        & \cite{broscheit-2019-investigating,logeswaran-etal-2019-zero,wu-etal-2020-scalable}
        & 
        \\ 
    \midrule 
    \multirow{3}{*}{Relation classification} 
        & 
        TACRED \cite{zhang-etal-2017-position},
        FewRel \cite{han-etal-2018-fewrel}
        &&
        & \cite{zhang-etal-2019-ernie,yamada-etal-2020-luke,poerner-etal-2020-e-bert}
        & \cite{baldini-soares-etal-2019-matching,bouraoui-etal-2020-inducing}
        \\ 
    \midrule 
    % \multirow{4}{*}{Relation classification} &
    % \midrule 
    \multirow{3}{*}{Compositional reasoning} 
        & 
        Synthetic \cite{kassner-etal-2020-pretrained,clark-etal-2020-transformers} or semi-synthetic \cite{talmor-etal-2020-leap,thorne-etal-2021-database}
        && 
        \cite{kassner-etal-2020-pretrained}
        & 
        & \cite{clark-etal-2020-transformers,talmor-etal-2020-leap,talmor-etal-2020-olmpics,thorne-etal-2021-database} \\ 
    \midrule 
    \multirow{4}{*}{Question answering} 
        & WebQuestions \cite{berant-etal-2013-semantic},
        SQuAD \cite{rajpurkar-etal-2016-squad},
        TriviaQA \cite{joshi-etal-2017-triviaqa}, CommonsenseQA \cite{talmor-etal-2019-commonsenseqa}
        && \cite{tamborrino-etal-2020-pre,shwartz-etal-2020-unsupervised} 
        & 
        \cite{broscheit-2019-investigating,roberts-etal-2020-much,fevry-etal-2020-entities,yamada-etal-2020-luke,de-cao-2021-autoregressive}
        & \cite{ye-etal-2020-align-mask,ma-etal-2021-knowledge-driven,verga-etal-2020-facts}  \\ 
    \midrule 
    \multirow{3}{*}{\kb{} construction} 
        & 
        FB15K-237 \cite{toutanova-chen-2015-observed},
        ConceptNet \cite{li-etal-2016-commonsense},
        ATOMIC \cite{sap-etal-2019-atomic}
        && 
        \cite{davison-etal-2019-commonsense}
        & 
        \cite{shen-etal-2020-exploiting}
        &
        \cite{yao-etal-2019-kg-bert, bosselut-etal-2019-comet,hwang-etal-2021-comet-atomic} \\ 
    \bottomrule
\end{tabular}
}
% \vspace{-.3cm}
\end{table*}
